SCoDA: Domain Adaptive Shape Completion for Real Scans

3D shape completion from point clouds is a challenging task, especially from scans of real-world objects. Considering the paucity of 3D shape ground truths for real scans, existing works mainly focus on benchmarking this task on synthetic data, e.g. 3D computer-aided design models. However, the domain gap between synthetic and real data limits the generalizability of these methods. Thus, we propose a new task, SCoDA, for the domain adaptation of real scan shape completion from synthetic data. A new dataset, ScanSalon, is contributed with a bunch of elaborate 3D models created by skillful artists according to scans. To address this new task, we propose a novel cross-domain feature fusion method for knowledge transfer and a novel volume-consistent self-training framework for robust learning from real data. Extensive experiments prove our method is effective to bring an improvement of 6%~7% mIoU.

==> figures/dataset_exh.tex <==
\begin{figure*}[ht!] \centering
    % \makebox[0.245\linewidth]{\scriptsize (a) Method 1}
    % \makebox[0.245\linewidth]{\scriptsize (b) Method 2}
    % \makebox[0.245\linewidth]{\scriptsize (c) Method 3}
    % \makebox[0.245\linewidth]{\scriptsize (d) Method 4}
    % \\
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0008_00_4.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0008_00_4_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0008_00_4_c.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0369_00_12.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0369_00_12_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0369_00_12_c.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0152_00_8.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0152_00_8_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0152_00_8_c.png}
    \\
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0054_00_60.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0054_00_60_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0054_00_60_c.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0329_00_7.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0329_00_7_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0329_00_7_c.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0235_00_16.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0235_00_16_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0235_00_16_c.png}
    \\
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0269_00_0.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0269_00_0_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0269_00_0_c.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0451_01_13.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0451_01_13_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0451_01_13_c.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0031_00_6.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0031_00_6_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0031_00_6_c.png}
    \\
    \includegraphics[width=0.126\linewidth]{figures/datasets/240.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/car_pcd_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/240_c.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0616_00_31.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0616_00_31_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0616_00_31_c.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0576_00_9.png}
    \includegraphics[width=0.126\linewidth]{figures/datasets/scene0576_00_9_m.png}
    \includegraphics[width=0.063\linewidth]{figures/datasets/scene0576_00_9_bed.png}
    \\
    \caption{Visualization of samples in our dataset.} 
    \label{fig:dataset_exh}
\end{figure*}

==> tables/figures4by4.tex <==
\begin{figure}[t] \centering
    \makebox[0.108\textwidth]{\scriptsize (a) Method 1}
    \makebox[0.108\textwidth]{\scriptsize (b) Method 2}
    \makebox[0.108\textwidth]{\scriptsize (c) Method 3}
    \makebox[0.108\textwidth]{\scriptsize (d) Method 4}
    \\
    \includegraphics[width=0.108\textwidth]{example-image}
    \includegraphics[width=0.108\textwidth]{example-image}
    \includegraphics[width=0.108\textwidth]{example-image}
    \includegraphics[width=0.108\textwidth]{example-image}
    \\
    \includegraphics[width=0.108\textwidth]{example-image}
    \includegraphics[width=0.108\textwidth]{example-image}
    \includegraphics[width=0.108\textwidth]{example-image}
    \includegraphics[width=0.108\textwidth]{example-image}
    \\
    \includegraphics[width=0.108\textwidth]{example-image}
    \includegraphics[width=0.108\textwidth]{example-image}
    \includegraphics[width=0.108\textwidth]{example-image}
    \includegraphics[width=0.108\textwidth]{example-image}
    \\
    \caption{A figure with text header.} 
    \label{fig:figure3}
\end{figure}

==> tables/one_table.tex <==
\begin{table}[tb]\centering
    \caption{Efficiency.}
    \label{tab:efficiency}
    \resizebox{0.4\textwidth}{!}{
    \large
    \begin{tabular}{*{10}{c}}
        \toprule
       Method & Storage (MB) &  FLOPs (M) & PSNR$\uparrow$ &  FLIP$\downarrow$ \\
        \midrule
        A    & 1 & 1 & 2 & 3  \\
        B    & 1 & 1 & 2 & 3  \\
        \midrule
        Ours & 1 & 2 & 3 & 4  \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/two_subtables.tex <==
\newcommand{\PSNRT}{PSNR\xspace}
\newcommand{\VQM}{HDR-VQM\xspace}
\newcommand{\VDP}{HDR-VDP2\xspace}
\newcommand{\LowExposure}{Low-Exposure\xspace}
\newcommand{\MiddleExposure}{Middle-Exposure\xspace}
\newcommand{\HighExposure}{High-Exposure\xspace}
\newcommand{\AllExposure}{All-Exposure\xspace}

\makebox[\textwidth]{\small (a) Results on dataset A.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & \Scnd{40.00} & 73.70 & \Scnd{40.04} & \Scnd{70.08} & \Scnd{40.02} & 71.89 & \Scnd{76.22} 
                  & \Scnd{39.61} & 73.24 & \Frst{39.67} & \Frst{73.24} & \Frst{40.01} & 67.90 & \Frst{39.77} & 70.37 & 79.55 \\
    Method B      & 34.54 & 80.22 & 39.25 & 65.96 & 36.90 & 73.09 & 65.33 
                  & 36.51 & 77.78 & 37.45 & 69.79 & 39.02 & 64.57 & 37.66 & 70.71 & 70.13 \\
    Method C  & 39.79 & \Scnd{81.02} & 39.96 & 67.25 & 39.88 & \Scnd{74.13} & 73.84 
                  & 39.48 & \Scnd{78.13} & 38.43 & 70.08 & 39.60 & \Scnd{67.94} & 39.17 & \Scnd{72.05} & \Scnd{80.70} \\
    Ours          & \Frst{41.95} & \Frst{81.03} & \Frst{40.41} & \Frst{71.27} & \Frst{41.18} & \Frst{76.15} & \Frst{78.84}
                  & \Frst{40.00} & \Frst{78.66} & \Scnd{39.27} & \Scnd{73.10} & \Scnd{39.99} & \Frst{69.99} & \Scnd{39.75} & \Frst{73.92} & \Frst{82.87} \\
    \bottomrule
\end{tabular}
}

\vspace{0.5em}
\makebox[\textwidth]{\small (b) Results on dataset B.} 
\resizebox{\textwidth}{!}{
    \Large
\begin{tabular}{l||*{2}{c}|*{2}{c}|*{3}{c}||*{2}{c}|*{2}{c}|*{2}{c}|*{3}{c}}
    \toprule
    & \multicolumn{7}{c||}{2-Exposure} & \multicolumn{9}{c}{3-Exposure} \\
    & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c||}{\AllExposure} & \multicolumn{2}{c}{\LowExposure} & \multicolumn{2}{c}{\MiddleExposure} & \multicolumn{2}{c}{\HighExposure} & \multicolumn{3}{c}{\AllExposure} \\
    Method & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \VQM & \PSNRT & \VDP & \PSNRT & \VDP  & \PSNRT & \VDP & \PSNRT & \VDP & \VQM \\
    \midrule
    Method A & 37.73 & 74.05 & 45.71 & 66.67 & 41.72 & 70.36 & 85.33 
                  & 37.53 & 72.03 & 36.38 & 65.37 & 34.73 & 62.24 & 36.21 & 66.55 & 84.43 \\
    Method B      & 36.41 & 85.68 & \Scnd{49.89} & \Scnd{69.90} & 43.15 & 77.79 & 78.92 
                  & 36.43 & 77.74 & 39.80 & \Scnd{67.88} & \Scnd{43.03} & \Scnd{64.74} & 39.75 & \Scnd{70.12} & 87.93 \\
    Method C  & \Scnd{39.94} & \Scnd{86.77} & 49.49 & 69.04 & \Scnd{44.72} & \Scnd{77.91} & \Scnd{87.16} 
                  & \Scnd{38.34} & \Scnd{78.04} & \Scnd{41.21} & 66.07 & 42.66 & 64.01 & \Scnd{40.74} & 69.37 & \Scnd{89.36}\\
    Ours          & \Frst{40.83} & \Frst{86.84} & \Frst{50.10} & \Frst{71.33} & \Frst{45.46} & \Frst{79.09} & \Frst{87.40} 
                  & \Frst{38.77} & \Frst{78.11} & \Frst{41.47} & \Frst{68.49} & \Frst{43.24} & \Frst{65.08} & \Frst{41.16} & \Frst{70.56} & \Frst{89.56}\\
    \bottomrule
\end{tabular}
}

